LeadCache: Regret-Optimal Caching in Networks

We consider an online prediction problem in the context of network caching. Assume that multiple users are connected to several caches via a bipartite network. At any time slot, each user may request an arbitrary file chosen from a large catalog. A user's request at a slot is met if the requested file is cached in at least one of the caches connected to the user. Our objective is to predict, prefetch, and optimally distribute the files on the caches at each slot to maximize the total number of cache hits. The problem is non-trivial due to the non-convex and non-smooth nature of the objective function. In this paper, we propose $\texttt{LeadCache}$ - an efficient online caching policy based on the Follow-the-Perturbed-Leader paradigm. We show that $\texttt{LeadCache}$ is regret-optimal up to a factor of $\tilde{O}(n^{3/8}),$ where $n$ is the number of users. We design two efficient implementations of the $\texttt{LeadCache}$ policy, one based on Pipage rounding and the other based on Madow's sampling, each of which makes precisely one call to an LP-solver per iteration. Furthermore, with a Strong-Law-type assumption, we show that the total number of file fetches under $\texttt{LeadCache}$ remains almost surely finite over an infinite horizon. Finally, we derive an approximately tight regret lower bound using results from graph coloring. We conclude that the learning-based $\texttt{LeadCache}$ policy decisively outperforms the state-of-the-art caching policies both theoretically and empirically.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}
%%%% BEGIN INSTRUCTIONS %%%
%The checklist follows the references.  Please
%read the checklist guidelines carefully for information on how to answer these
%questions.  For each question, change the default \answerTODO{} to \answerYes{},
%\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
%justification to your answer}, either by referencing the appropriate section of
%your paper or providing a brief inline description.  For example:
%\begin{itemize}
%  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%  \item Did you include the license to the code and datasets? \answerNA{}
%\end{itemize}
%Please do not modify the questions and only use the provided macros for your
%answers.  Note that the Checklist section does not count towards the page
%limit.  In your paper, please delete this instructions block and only keep the
%Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Section \ref{conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
	\item Did you include complete proofs of all theoretical results?
    \answerYes{See the supplementary material.}
\end{enumerate}

\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{The code is available at \url{https://github.com/AbhishekMITIITM/LeadCache-NeurIPS21}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{Please see Figure \ref{hit-download-rates}.}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See Section \ref{addl_plots} in the supplementary.}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{Included the full reference to the dataset used \citep{berger2018practical, trace}.}
  \item Did you mention the license of the assets?
    \answerYes{In Section \ref{experiments}, we mentioned that the dataset is available under a BSD 2-Clause License.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{Mentioned that we used an anonymized production trace. See Section \ref{experiments}.}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> randomizedrounding.tex <==
\paragraph{Randomized Rounding:}
It can be easily verified that we can replace the inequality constraint for finite cache capacity with equality. We now propose the following randomized rounding procedure which produces a feasible integral allocation while guaranteeing an objective value of at least $(1-1/e)\textsf{OPT}.$ 

\begin{algorithm}
\caption{\textsf{Randomized Rounding} for {\sc Caching Inelastic Contents}}
\label{randomized}
\begin{algorithmic}[1]
\STATE Solve the LP relaxation \eqref{LP_relax}. Let the optimal cache configuration be given by $\bm{y}=\big(y_f^j, j \in \mathcal{J}, f \in [N]\big).$
\STATE For each cache $j \in \mathcal{J},$ sample $C$ files independently at random with replacement.  During each sampling, a file $f \in [N]$ is selected with probability $\frac{y^j_f}{C}.$ 
\STATE Denote the resulting random output cache configuration by $\big(\tilde{Y}_f^j, j \in \mathcal{J}, f \in [N]\big)$. Set \[\tilde{Z}^i_f= \bigvee_{j \in \partial^+(i)}\tilde{Y}_f^j.\]
\end{algorithmic}
\end{algorithm}
We prove the following proposition: 
\begin{framed}
\begin{proposition}
	The randomized rounding scheme, given in Algorithm \ref{randomized} is an $(1-\frac{1}{e})$ approximation algorithm for the IP \eqref{LP_relax}.
\end{proposition}
\end{framed}
\begin{proof}

Clearly, with the above randomized sampling scheme, we have 
\[ \mathbb{P}(\tilde{Y}_f^j=0)= \bigg(1-\frac{y^j_f}{C}\bigg)^C. \]
%
%\begin{enumerate}
%\item  Solve the LP relaxation \eqref{LP_relax}. Let the optimal  (non-integral) cache allocation be given by $\bm{y}=\big(y_f^j, j \in \mathcal{J}, f \in [N]\big).$
%\item For each cache $j \in \mathcal{J},$ sample $C$ files independently at random with replacement.  At each sampling, the file $f \in [N]$ is selected with probability $\frac{y^j_f}{C}.$ Denote the random output cache configuration by $\big(\tilde{Y}_f^j, j \in \mathcal{J}, f \in [N]\big)$ Hence, 
%\[ \mathbb{P}(\tilde{Y}_f^j=0)= \bigg(1-\frac{y^j_f}{C}\bigg)^C. \]
%We set $\tilde{Z}^i_f= \bigvee_{j \in \partial^+(i)}\tilde{Y}_f^j.$ 
%\end{enumerate}
Now, consider any variable $z^i_f$ in  \eqref{LP_relax}. We consider two different cases:
\paragraph{\textsf{Case-I}: $z^i_f=1$ in the optimal solution:}  Since $\tilde{Z}^i_f= \bigvee_{j \in \partial^+(i)}\tilde{Y}_f^j,$ we have that 
\begin{eqnarray*}
 \mathbb{P}(\tilde{Z}^i_f=1) &\stackrel{(a)}{=}& 1- \prod_{j \in \partial^+(i)} \mathbb{P}(\tilde{Y}_f^j=0) \\
 &=& 1 - \prod_{j \in \partial^+(i)} \bigg(1-\frac{y^j_f}{C}\bigg)^C\\
 &\stackrel{(b)}{\geq} & 1 - \exp(-\sum_{j \in \partial^+(i)} y^j_f)\\
 &\stackrel{(c)}{\geq}& 1 - \frac{1}{e}, 
\end{eqnarray*}
where the inequality (a) follows from the fact that the collection of the r.v.s $\{\tilde{Y}^j_f\}_{1 \leq f \leq N}$ are independent, the inequality (b) follows from the standard inequality $e^x \geq 1+x, \forall x \in \mathbb{R}$, and the inequality (c) follows from the fact that since $z_i^f=1$, it must be that $\sum_{j \in \partial^+(i)}y_f^j \geq 1.$
\paragraph{Case-II: $z^i_f<1$ in the optimal solution:} In this case, we must have
\begin{eqnarray}\label{min_val} 
 z^i_f = \sum_{j \in \partial^+(i)}y^j_f <1.
\end{eqnarray}
Now, since $\tilde{Z}^i_f= \bigvee_{j \in \partial^+(i)}\tilde{Y}_f^j$, using the same argument as in Case-I, we have 
\begin{eqnarray*} 
 \mathbb{P}(\tilde{Z}^i_f=1) &=& 1 - \prod_{j \in \partial^+(i)}\bigg(1-\frac{y^j_f}{C}\bigg)^C\\
 &\geq & 1 - \exp(-\sum_{j \in \partial^+(i)} y^j_f)\\
 &\stackrel{(a)}{=}& 1- \exp(-z^{i}_f)\\
 &\stackrel{(b)}{\geq}& (1-\frac{1}{e})z^{i}_f.
 \end{eqnarray*}
where the inequality (a) follows from Eqn.\ \eqref{min_val} and the inequality (b) follows from the fact that 
\begin{eqnarray*}
1-\exp(-x)\geq \big(1-\frac{1}{e}\big)x, ~~0\leq x \leq 1.	
\end{eqnarray*}
The above inequality follows from the fact that the function $f(x)\equiv 1-\exp(-x)$ is concave, and hence for all $0 \leq x \leq 1$, the function $f(x)$ is lower bounded by the straight line connecting the points $(0, f(0))$ and $(1, f(1)).$
 
 Combining Case-I and Case-II, we conclude that for all cases, we have the following bound: 
 \begin{eqnarray*}
 \mathbb{E}(\tilde{Z}^i_f) \geq (1-\frac{1}{e})z^i_f, ~~\forall i,f.	
 \end{eqnarray*}
 Finally, using the linearity of expectation, we conclude that the randomized rounding procedure yields a feasible cache configuration which ensures the following objective value in expectation:
 \begin{eqnarray*}
 \mathbb{E}\langle \bm \Theta, \bm{\tilde{Z}}\rangle = \sum_{i \in \mathcal{I}} \langle \bm{\theta}^i, \mathbb{E}(\bm{\tilde{Z}}^i) \rangle)\geq (1-\frac{1}{e})\textsf{OPT}.	
 \end{eqnarray*}
\end{proof}




